Knowledge Mechanisms in Large Language Models: A Survey and Perspective

Understanding knowledge mechanisms in Large Language Models (LLMs) is crucial for advancing towards trustworthy AGI. This paper reviews knowledge mechanism analysis from a novel taxonomy including knowledge utilization and evolution. Knowledge utilization delves into the mechanism of memorization, comprehension and application, and creation. Knowledge evolution focuses on the dynamic progression of knowledge within individual and group LLMs. Moreover, we discuss what knowledge LLMs have learned, the reasons for the fragility of parametric knowledge, and the potential dark knowledge (hypothesis) that will be challenging to address. We hope this work can help understand knowledge in LLMs and provide insights for future research.

==> cr_section/cr_Application.tex <==
\section{Application of Knowledge Mechanism}
\label{Application}
The mechanism analysis of knowledge utilization and evolution may provide an avenue to construct more efficient and trustworthy models in practice.




\subsection{Efficient LLMs}
\label{Efficient LLMs}

Researchers have been working to reduce the cost of training and inference for LLMs through various optimization strategies, including architecture \cite{DBLP:conf/emnlp/AinslieLJZLS23,DBLP:journals/jmlr/FedusZS22}, data quality \cite{DBLP:journals/corr/abs-2304-08442}, parallelization \cite{DBLP:journals/corr/abs-2401-10241}, generalization theory \cite{DBLP:journals/corr/abs-2405-05409}, hardware \cite{DBLP:journals/corr/abs-2304-03208}, scaling laws \cite{DBLP:journals/corr/abs-2203-15556}, optimizer \cite{DBLP:journals/corr/abs-2305-14342}, etc.
The underlying knowledge mechanisms offer LLMs new potential for efficiently storing, utilizing, and evolving knowledge.

For \textbf{knowledge storage and utilization} in LLMs, \textit{knowledge (memory) circuit} provides the theory to decompose the knowledge computations of an LLM into smaller, recurring parts \cite{ExplicitMemory}.
These smaller parts guide the determination of which types of knowledge should be encoded into parameters. 
Therefore, $\text{Memory}^3$ \cite{ExplicitMemory} designs an explicit memory mechanism for Transformer-based LLMs, alleviating the burden of parameter size.
Specifically, $\text{Memory}^3$ designs external information, explicit memory, and implicit memory for different usage frequencies, reducing writing and reading costs.
% For \textbf{knowledge utilization}, editing technologies aim to precisely manipulate (insert, update and erase) specific knowledge with small data and computational resources \footnote{The details of editing technologies can be found in \S \ref{Group Evolution}.}.
For \textbf{knowledge evolution}, the knowledge mechanism analysis inspires \textit{editing} and \textit{model merging}.
The details of editing technologies can be found in \S \ref{Group Evolution}.
Model merging technologies \footnote{Model merging also includes methods that directly interpolation \cite{DBLP:journals/corr/abs-2403-13257} or randomly fusing \cite{DBLP:journals/corr/abs-2311-03099}, ignoring parameter directions. These methods are naive and are not the focus of our discussion here.} leverage parameter directions to combine multiple task-specific models into a single multitask model without performing additional training rather than training from scratch.
For instance, 
Task Arithmetic \cite{DBLP:conf/iclr/IlharcoRWSHF23} identifies the weight directions of task capabilities in different models, and then integrates a more powerful model by arithmetic operations on weight directions.
TIES \cite{DBLP:conf/nips/YadavTCRB23} resolves parameters directions conflicts, and merges only the parameters that are in alignment with the final agreed-upon sign.
\citet{DBLP:journals/corr/abs-2403-13187} further propose evolutionary optimization of model merging, which automatically discovers effective combinations of open-source models, harnessing their group intelligence without requiring extensive training data or computational resources.
Besides, the Lottery Ticket Hypothesis \cite{DBLP:conf/iclr/FrankleC19} provides a cornerstone for \textit{model compression}, generalizing across various datasets, optimizers, and model architectures \cite{DBLP:conf/nips/MorcosYPT19,DBLP:conf/nips/ChenCWGLW21}.
However, model compression often limits the success of editing and model merging \cite{kolbeinsson2024composable}.
This phenomenon poses challenges for practical implementations, highlighting the need for more effective strategies.








\subsection{Trustworthy LLMs}
\label{Trustworthy LLMs}

% Investigating the causal relationships between inputs and outputs of LLMs contributes to enhancing their safety and reliability.
Numerous studies investigate the underlying causes of security risks \cite{reuel2024open,ren2024safetywashing,li2024more,bengio2024government,bengio2024managing,DBLP:journals/corr/abs-2405-06624}.
In particular,
\citet{DBLP:conf/nips/0001HS23} delve into the safety of LLM and reveal that the success of jailbreak is mainly due to the distribution discrepancies between malicious attacks and training data.
\citet{DBLP:conf/emnlp/GevaCWG22} and \citet{DINM} further discover that some parameters within LLMs, called toxic regions, are intrinsically tied to the generation of toxic content. 
\citet{ji2024language} even conjecture that LLMs resist alignment.
Therefore, traditional aligned methods, DPO \cite{DBLP:conf/nips/RafailovSMMEF23} and SFT, seem to merely bypass toxic regions \cite{DBLP:journals/corr/abs-2401-01967,DINM}, making them susceptible to other jailbreak attacks \cite{DBLP:journals/corr/abs-2311-09096}.




Inspired by the knowledge mechanism analysis in LLMs, a promising trustworthy strategy may be \textbf{designing architecture and training process} during the pre-training phase to encouraging modularity \cite{DBLP:journals/entropy/LiuGT24,DBLP:journals/corr/abs-2310-07711}, sparsity \cite{DBLPconf/icml/ChughtaiCN23}, and monosemanticity \cite{Monosemanticity,DBLP:journals/corr/abs-2211-09169}, which make the reverse engineering process more tractable \cite{DBLP:journals/corr/abs-2211-09169,Monosemanticity,DBLP:journals/entropy/LiuGT24,DBLP:journals/corr/abs-2310-17230}.
Yet, maintaining sparsity for a vast amount of world knowledge requires substantial resources, and whether monosemantic architecture can support advanced intelligence remains elusive.
Besides, \textbf{machine unlearning} \cite{nguyen2022survey,tian2024forget,DBLP:journals/corr/abs-2310-10683} aims to forget privacy or toxic information learned by LLMs. 
However, these unlearning methods suffer overfitting, forgetting something valuable due to the difficulty of disentangling verbatim memorization and general capabilities \cite{VerbatimMemorization,DBLP:journals/corr/abs-2404-02062}.
Another alternative technique is \textbf{knowledge editing}, precisely modifying LLMs using few instances during the post-training stage \cite{DBLP:journals/corr/abs-2310-19704,yao-etal-2023-editing,DBLP:journals/corr/abs-2310-16218,Fundamental,DBLP:journals/corr/abs-2402-19465}.
Extensive experiments demonstrate that knowledge editing has the potential to detoxify LLMs \cite{DBLP:journals/corr/abs-2402-13462}.
Specifically, \cite{DBLP:conf/emnlp/WuLXDW0X23} and \citet{DBLP:conf/emnlp/GevaCWG22} deactivate the neurons related to privacy information and toxic tokens, respectively.
\cite{DINM} identify and then erases toxic regions in LLMs. 
However, knowledge editing also introduces side effects, such as the inability of the modified knowledge to generalize to multi-hop tasks \cite{DBLP:conf/emnlp/ZhongWMPC23,DBLP:journals/corr/abs-2310-02129,DBLP:journals/corr/abs-2307-12976,kong2024aligning} and the potential to impair the model's general capabilities \cite{DBLP:journals/corr/abs-2401-04700,HengJi}. 
Therefore, recent efforts focus on \textbf{representation editing} instead of editing parameters in knowledge editing \cite{RepresentationEngineering,DBLP:journals/corr/abs-2308-10248,AlignmentHiddenStates,Beliefs}.
These representations (hidden states) within LLMs can trace and address a wide range of safety-relevant problems, including honesty, harmlessness, and power seeking.
Later, \cite{ReFT} develop a family of representation finetuning methods to update new knowledge. \cite{CircuitBreakers} propose circuit-breaking \cite{DBLP:journals/corr/abs-2309-05973}, directly controlling the representations that are responsible
for harmful outputs.
However, these representation editing strategies require meticulous hyperparameter tuning for each task. More efficient optimization methods are needed to align with computational or temporal constraints.




==> cr_section/cr_Conclusion.tex <==


\section{Conclusion}
\label{Conclusion}
In this paper, we propose a novel knowledge mechanism analysis taxonomy and review knowledge evolution. 
We further discuss knowledge utilization issues, as well as unexplored dark knowledge.
We hope these insights may inspire some promising directions for future research and shed light on more powerful and trustworthy models.



% In this paper, we propose a novel knowledge mechanism analysis taxonomy and review knowledge evolution within individual and groups. 
% We further discuss the acquired and misused knowledge, as well as unexplored dark knowledge within LLMs.
% We hope these insights may inspire some promising directions for future research and shed light on more powerful and trustworthy models.

% in \S \ref{Future_Directions} 

==> cr_section/cr_Discussion.tex <==



\section{Discussion}
\label{Discussion}
In this section, we discuss some open questions and seek to explore their essence and underlying principles.
Specifically, 
we discuss what knowledge LLMs have learned in \S \ref{Learned}, 
examine the fragility of the learned knowledge in application in \S \ref{Challenges}, 
analyze the dark knowledge not yet learned by machines or humans in \S \ref{Dark Knowledge}, 
and explore how LLMs can expand the boundaries of unknown knowledge from interdisciplinary perspectives \S \ref{How to benefit from interdisciplinarity?}.






\subsection{What Knowledge Have LLMs Learned?}
\label{Learned}

\textit{Critics question whether LLMs truly have knowledge} or if they are merely mimicking \cite{DBLP:journals/corr/abs-2404-15146}, akin to the ``Stochastic Parro'' \cite{DBLP:conf/fat/BenderGMS21} and ``Clever Hans'' \cite{DBLP:conf/eacl/ShapiraLAZCGSS24}.
We first review the doubts from the following three levels through \textit{observation phenomena}:
1) Memorization: LLMs primarily rely on positional information over semantic understanding \cite{DBLP:conf/acl/LiLSDSLJJL22} to predict answers.
Additionally, LLMs may generate different answers for the same question due to different expressions.
2) Comprehension and application: \citet{DBLP:journals/corr/abs-2309-14402} argue that LLMs hardly efficiently apply knowledge from pre-training data, even when such knowledge is perfectly stored and fully extracted from LLMs.
Therefore, LLMs struggle with various reasoning tasks \cite{DBLP:journals/corr/abs-2307-02477,Alice,DBLP:journals/corr/abs-2405-14831} as well as the reversal curse \cite{DBLP:journals/corr/abs-2309-12288}. 
Besides, LLMs are not yet able to reliably act as text world simulators and encounter difficulties with planning \cite{Simulators}.
3) Creation: Although LLMs are capable of generating new terms, their quality often falls below that created by humans \cite{DBLP:journals/cacm/Raiola23}. 
Even though LLMs possess knowledge, some critics argue that current \textit{analysis methods} may only explain low-level co-occurrence patterns, not internal mechanisms.
The primary criticism asserts that the components responsible for certain types of knowledge in LLM fail to perform effectively in practical applications \cite{DBLP:conf/nips/HaseBKG23}. 
In addition, the components responsible for specific knowledge within LLMs vary under different methods. 
For these criticisms, \citet{DBLP:journals/corr/abs-2402-13731,DBLP:conf/aaai/ChenCCLZ24} propose degenerate neurons and posit that different degenerate components indeed independently express a fact.
\citet{Query} delineate the differences in the mechanisms of knowledge storage and representation, proposing the Query Localization Assumption to response these controversies.
\citet{DBLP:journals/corr/abs-2309-14316} further observe that knowledge may be memorized but not extracted due to the knowledge not being sufficiently augmented (e.g., through paraphrasing, sentence shuffling) during pretraining.
Hence, rewriting the training data to provide knowledge augmentation and incorporating more instruction fine-tuning data in the pre-training stage can effectively alleviate the above challenges and criticisms.


Despite considerable criticism, the mainstream view \cite{DBLP:journals/corr/abs-2405-12205,jinemergent,jin2024latent} is that \textbf{current LLMs may possess basic world knowledge via memorization but hardly master underlying principles for reasoning and creativity}.
In other words, LLMs master basic knowledge via memorization (discussed in \S \ref{Memorization}). 
Although LLMs possess the foundational ability to comprehend and apply knowledge (discussed in \S \ref{Comprehension and Application}), exhibiting plausible and impressive reasoning capabilities.
Current LLMs still struggle with reasoning and planning in complex tasks due to the fragility of knowledge in LLMs (elaborated in \S \ref{Challenges}). 
These reasoning and planning abilities usually require to be induced through techniques such as ICL and CoT.
Unfortunately, current LLMs are nearly incapable of creation due to the architectural limitations (discussed in \S \ref{Creation}).
Therefore, some scholars explore various architectural choices (e.g., Mamba \cite{DBLP:journals/corr/abs-2312-00752}) and training procedures.
Besides, recent research attempts to manipulate neurons, knowledge circuits, or representations \cite{DBLP:journals/corr/abs-2309-14402,RepresentationEngineering,ReFT,DBLP:conf/nips/0002PVPW23} to explore more knowledge and awaken the reasoning and planning capabilities of LLMs.


\noindent \textbf{\includegraphics[scale=0.15]{fig/remark.png} Remarks}: LLMs have learned basic knowledge of the world by \textit{momorization}.
However, the learned knowledge is fragile, leading to challenges in \textit{knowledge comprehension and application}.
Unfortunately, due to architectural limitations, current LLMs struggle with \textit{creation}.



% but encounter challenges in application (\S \ref{Challenges}). 
% Some knowledge still lies beyond their current cognitive scope (\S \ref{Dark Knowledge}).
% For example, due to architectural limitations, LLMs struggle with creativity.






% How can we enable LLMs to learn more knowledge and become more intelligent?
% Recent research attempts to manipulate neurons, knowledge circuits, or representations \cite{RepresentationEngineering,ReFT,DBLP:conf/nips/0002PVPW23}.




% \subsection{Improper Learning or Misuse?}
\subsection{Why Is Learned Knowledge Fragile?}
\label{Challenges}
% \todo{add evolution and xxx}
% \见风使舵
% 精神错乱，多重人格
% LLM知道input是虚假的，有真理的时候才坚定
% 对齐 的方法在幻觉中的作用，maybe 在某个区域控制 模型知识自己不知道
% 人类测谎仪
\textit{The knowledge learned by LLMs is fragile}, leading to challenges in application including hallucination, knowledge conflicts, failed reasoning, and safety risk \footnote{The secure risk is elaborated in \S \ref{Trustworthy LLMs}.}.
\textbf{Hallucination} denotes content generated by LLMs that diverges from real-world facts or inputs \cite{DBLP:journals/corr/abs-2311-05232,DBLP:journals/corr/abs-2401-11817,farquhar2024detecting,chen2024multi}.
On the one hand, factuality hallucination underscores the disparity between generated content and real-world knowledge.
% , often characterized by factual inconsistencies or fabrication.
On the other hand, faithfulness hallucination describes the departure of generated content from user instructions or input context, as well as the coherence maintained within the generated content.
\textbf{Knowledge Conflict} inherently denotes inconsistencies in knowledge \cite{DBLP:journals/corr/abs-2403-08319,DBLP:journals/corr/abs-2404-16032}.
On the one hand, internal memory conflicts within the model cause LLMs to exhibit unpredictable behaviors and generate differing results to inputs which are semantically equivalent but syntactically distinct \cite{DBLP:journals/corr/abs-2403-08319,DBLP:journals/corr/abs-2310-07521,DBLP:journals/corr/abs-2311-05876,DBLP:journals/corr/abs-2211-05853}.
% \citet{DBLP:conf/nips/0002PVPW23} even discover that the correct knowledge is indeed stored in LLM, but it may not be accurately utilized in related tasks.
% \citet{knowledgecircuit} further
On the other hand, context-memory conflict emerges when external context knowledge contradicts internal parametric knowledge \cite{DBLP:journals/corr/abs-2403-08319,DBLP:conf/acl/MallenAZDKH23}.


We posit that \textbf{these challenges mainly derive from improper learning data.}
Specifically, {hallucination} is introduced by data \cite{DBLP:conf/emnlp/KangC23,ExtrinsicHallucinations,zhang2024knowledge}, heightened during the pre-training \cite{DBLP:conf/nips/BrownMRSKDNSSAA20,DBLP:conf/acl/0001C22}, alignment \cite{DBLP:journals/corr/abs-2304-13734,DBLP:conf/nips/Ouyang0JAWMZASR22}, and deficiencies in decoding strategies \cite{DBLP:conf/acl/LewisDF18,DBLP:journals/corr/abs-2309-03883,DBLP:journals/corr/abs-2305-14739}.
Internal memory conflict can be attributed to training corpus bias \cite{DBLP:conf/emnlp/WangMWZC23}, and exacerbated by decoding strategies \cite{DBLP:conf/nips/LeePXPFSC22} and knowledge editing.
Context-memory conflict arises mainly from the absence of accurate knowledge during training, necessitating retrieval from databases and the Web.
Failed reasoning usually arises from improper \textbf{data distribution}.
Specifically, knowledge may be memorized but not extractable or applicable without sufficient augmentation (e.g., through paraphrasing, sentence shuffling) during pre-training \cite{DBLP:journals/corr/abs-2309-14316}.
\citet{GeneralizationMemorization} also delve into the mechanism between parametric knowledge and learning data, demonstrate that training data distribution qualitatively influences generalization behavior \cite{jiang2024taia}.
\citet{Grokked} further suggest that improper data distribution in the corpus causes LLMs to lack essential reasoning components, such as the bridge layer for two-hop reasoning.
Similar mechanism analysis also supports the above conclusion, indicating that hallucinations arise from a lack of mover heads \cite{knowledgecircuit,DBLP:journals/corr/abs-2403-18167}, while knowledge conflicts stem from circuit competition failure in the last few layers \cite{DBLP:journals/corr/abs-2403-19521,merullo2023mechanism,DBLP:conf/nips/HaseBKG23,DBLP:conf/coling/Ju0DYRL24,DBLP:journals/corr/abs-2402-18154}.
% , claim that transformed-based models can't encapsulate or enhance knowledge related to reasoning into specific components, e.g., bridge layer, 
% That is, they lack specific retrieval heads, and the bridge layer is an internal factor leading to illusions and knowledge conflicts in LLMs.
Additionally, \textbf{data quantity} is crucial for knowledge robustness.
Specifically, LLMs can systematically learn comprehensive understandings of the world from extensive datasets, while little data during post-training stage may compromise the robustness of knowledge representation.
This assumption is confirmed by numerous failures of post-training.
For example, SFT exacerbates hallucinations \cite{DBLP:journals/corr/abs-2405-05904,DBLP:journals/corr/abs-2403-05612}, and knowledge editing amplifies knowledge conflicts \cite{DBLP:journals/corr/abs-2310-02129,DBLP:journals/corr/abs-2402-09656}.
Note that {safety issues} usually caused by the distribution of unseen data (adversarial input) \cite{DBLP:conf/nips/0001HS23,DBLP:journals/corr/abs-2401-06824}, which is elaborated in \S \ref{Trustworthy LLMs}.

\noindent \textbf{\includegraphics[scale=0.15]{fig/remark.png} Remarks}: Improper learning caused by data distribution and quantity might be the fundamental and primary cause.

% \noindent \textbf{\includegraphics[scale=0.15]{fig/remark.png} Remarks}: The knowledge fragility of LLMs may be attributed to misuse \cite{HallucinationStates,zhang2024knowledge}, but improper learning might be the fundamental and primary cause.



% \subsection{Dark Knowledge Hypothesis for LLMs?} 
\subsection{Does Difficult-to-Learn ``Dark Knowledge'' Exist?}
\label{Dark Knowledge}

The distribution and quality of data are vital for knowledge acquisition and robust operation within the model (machine).
Imagine an ideal scenario where we have access to all kinds of data to train the machine.
% Could these models achieve human-like intelligence?
The data includes all possible modalities, such as text, image, audio, video, etc.
Models can also interact with each other and the external environment.
In this long-term development, will there still be unknown dark knowledge for intelligence to human or model (machine)?


We hypothesize that there will still \textbf{exist dark knowledge for intelligence} in the future.
As shown in Fig \ref{fig:dark}, dark knowledge describes knowledge unknown to human or machine from the following three situations:
1) knowledge unknown to human \& known to machine (UH, KM).
Machines leverage vast amounts of data to explore internal patterns, whereas humans struggle with processing such data due to physiological limitations on data processing capacity and computational limits \cite{DBLP:journals/corr/abs-2312-09390,LLMCritics}. (UH, KM) includes gene prediction, intelligent transportation systems, and more.
Specifically, the structural elucidation of proteins remains mysterious to humans for a long time.
Cryo-electron microscopy, through capturing millions of images, first reveals the three-dimensional structures of proteins. 
Now, neural models can directly predict protein properties with high efficiency and accuracy \cite{pak2023using}.
2) knowledge known to human \& unknown to machine (UH, KM).
On the one hand, some scholars claim that machine can possess a ``Theory of Mind'' capability \cite{Beliefs} and emotions \cite{DBLP:conf/vr/NormoyleSD24}.
On the other hand, critics contend that machine lacks sentience \cite{DBLP:journals/socomp/AlveroP23} and merely probabilistically generates tokens.
The causes, extent, and dynamics of these emotions and sentience (like hunger, happiness, and loneliness) are subtle and intricate, making precise mathematical modeling by the machine exceptionally challenging.
Specifically, different factors are tightly coupled, making it nearly impossible to disentangle clear input-output relationships as with well-defined factual knowledge.
The sentient knowledge also exhibits chaotic behavior \cite{DBLP:journals/access/LiZY20a,DBLP:journals/complexity/DebboucheOBGKJA21}, being highly sensitive to initial conditions, where small changes can lead to vastly different outcomes \cite{DBLP:conf/complexnetworks/Segretain0TG20}.
% critics contend that machine lacks sentience and merely probabilistically generates tokens \cite{Simulators}.
% Specifically, 
% Specifically, some abstract knowledge like hunger, happiness, loneliness, and others cannot be fully represented by discrete data points.
% The above knowledge akin to NP-hard problems \cite{hochba1997approximation}, is also exceedingly complex and nearly impossible to model perfectly with current algorithms.
Therefore, opponents argue that no matter how many parameters machine possesses, it cannot learn all the knowledge that human has mastered.
3) knowledge unknown to human \& unknown to machine (UH, UM) is beyond our cognition, e.g., the uncertainty in quantum mechanics and the origin of the universe.
Generally, Dark knowledge extends beyond current data and model architectures \cite{GoAIs}.
(UH, UM) necessitates human-machine collaboration.
Yet, there is no definitive conclusion on whether (UH, KM) and (KH, UM) will be solved by model architecture, training data, and computational resources.
Note that plain knowledge known to human and machine in Fig \ref{fig:dark} encompasses well-defined historical events, mathematical theorems, physical laws, etc. 

\begin{figure}[!t]
    \centering
    \includegraphics[width=0.5\textwidth]{fig/dark.pdf}
    \caption{The future cognition of knowledge. The direction of the arrow represents the transition of knowledge from known to unknown.
    Dark knowledge, represented in gray, denotes knowledge unknown to human or machine.
    Plain knowledge known to both human and machine is highlighted in blue.
    }
    \label{fig:dark}
    \vskip -0.1in
\end{figure}

\noindent \textbf{\includegraphics[scale=0.15]{fig/remark.png} Remarks}: Dark knowledge may persist for a long time and requires human-machine collaboration to explore. 

\subsection{How to Explore More Knowledge from Interdisciplinary Inspiration?}
\label{How to benefit from interdisciplinarity?}
% How can LLMs continuously narrow the boundaries of dark knowledge and emerge with higher levels of intelligence?
% Continuous knowledge acquisition occurs throughout the human lifespan. Moreover, the human brain adeptly processes extensive multimodal information and efficiently stores and utilizes this knowledge. Can LLMs derive inspiration from interdisciplinary studies of human knowledge to advance the next generation of artificial intelligence?

How can LLMs continuously narrow the boundaries of dark knowledge and achieve higher level intelligence by leveraging the human experience of perpetual knowledge exploration throughout history? 
We may draw inspirations from the following interdisciplinary studies.


\noindent \textbf{Neuroscience} studies the structure and function of the brain at molecular, cellular, neural circuit, and neural network levels \cite{squire2012fundamental}.
Generally, both mechanism analysis in LLMs and neuroscience utilize observation and intervention methods to investigate the basic principles of knowledge learning and memory, decision-making, language, perception, and consciousness.
The biological signals of the human brain and the internal activation signals in LLMs are capable of reciprocal transformation \cite{caucheteux2023evidence, feng2023aligning,TransformerDebugger,flesher2021brain}.
Benefiting from advancements in neuroscience \cite{jamali2024semantic,thiebaut2022emergent,lee2022solving}, mechanism analysis in LLMs has identified analogous function neurons and regions \cite{functionregion}, and knowledge circuits \cite{knowledgecircuit}. 
Besides, leveraging plasticity theory in neuroscience, LLMs explain the underlying technical support for intelligence \cite{DBLP:journals/corr/abs-2403-06996}.
In the future, mechanism analysis of LLMs may draw inspirations from neuroscience, guiding the next generation of artificial intelligence in organizing neural frameworks and in the storage and utilization of knowledge \cite{ren2024brain,PNN,ExplicitMemory}.


\noindent \textbf{Cognitive Science} focuses on the mind and its processes \cite{kolak2006cognitive,baronchelli2013networks}, which include language, perception, memory, attention, reasoning, emotion and mental state.
Although cognitive science and neuroscience overlap in their research content, cognitive science focuses more on abstract knowledge such as mental states and emotions rather than specific knowledge.
Therefore, \citet{Beliefs} track beliefs of self and others (formulated as ``Theory of Mind'') in LLMs from the psychological perspective within cognitive science.
\cite{DBLP:conf/iclr/WangZX022} further observe social-cognitive skill in multi-agent communication and cooperation.
Generally, there is potential to explore advanced cognitive capabilities in LLMs from the perspective of cognitive science \cite{PositionPaper}.

\noindent \textbf{Psychology} is the scientific study of mind and behavior, which include both conscious and unconscious phenomena, and mental processes such as thoughts, feelings, and motives.
Benefiting from decades of research in human psychology, machine psychology aims to uncover mechanisms of decision-making and reasoning in LLMs by treating them as participants in psychological experiments \cite{DBLP:journals/corr/abs-2303-13988}.
Machine psychology may delve into mysteries of social situations and interactions
shaping machine behavior, attitudes, and beliefs \cite{DBLP:conf/uist/ParkOCMLB23}.
Besides, group psychology paves an auspicious path for exploring dynamics such as debates and collaboration among LLMs (agents).
For instance, \textit{Dunning–Kruger effect} \cite{DBLP:conf/cogsci/MahmoodiAB13,DBLP:conf/acsos/BrownE20} in cognitive psychology filed describes that individuals with limited competence in a particular domain overestimate their abilities, and vice versa.
This phenomenon may guide the final vote in group debates and discussions.
Promisingly, psychology of learning can be applied to study prompt designs, boost learning efficiency, improve communication strategies, and develop feedback mechanisms for LLMs \cite{DBLP:journals/corr/abs-2401-10904}. 


\noindent \textbf{Education} is the transmission of knowledge, skills, and character traits and manifests in various forms. 
Inspired by education in humans, \citet{DBLP:journals/corr/abs-2401-01286} categorize knowledge acquisition in LLMs into three distinct phases: recognition, association, and mastery. 
Besides, education instructs humans managing various types of conflicts: identifying inconsistencies in external information (inter-context conflict), deciding between external sources and internal memory (context-memory conflict), resolving memory confusion (internal memory conflict), and addressing cultural conflicts.
The above knowledge conflicts and integration also exist in knowledge evolution of LLMs across individuals and groups \cite{DBLP:journals/corr/abs-2308-02773}.
Fortunately, education facilitates humans in learning to learn.
Can LLMs similarly self-evolve to continuously adapt to societal changes and requirements?


\noindent \textbf{\includegraphics[scale=0.15]{fig/remark.png} Remarks}:
LLMs may improve their architecture and mechanisms for knowledge learning, storage, and expression, drawing inspiration from neuroscience. 
Besides, cognitive science and psychology provide promising alternatives for sophisticated intelligence, emergent capabilities and behaviors in evolution.
Educational studies can inspire the learning strategy of LLMs, navigating conflicts and integrating knowledge during their evolution.


% LLMs might acquire sophisticated intelligence from cognitive science.
% integration in individual and group LLMs evolution through insights from educational studies.

% Machine Psychology: Investigating Emergent Capabilities and Behavior in Large Language Models Using Psychological Methods.

==> cr_section/cr_Evolution.tex <==
\section{Knowledge Evolution in LLMs}
\label{Knowledge Evolution}

Knowledge in LLMs should evolve with changes in the external environment. We introduce the Dynamic Intelligence Hypothesis for knowledge evolution in individuals and groups.

\begin{bluebox}[Hypothesis 5: Dynamic Intelligence]

Conflict and Integration Coexist in the Dynamic Knowledge Evolution of LLMs.
%The evolution of knowledge in LLMs necessitates striking a balance between conflicting knowledge encountered at both the individual model level and through interactions with counterpart models or data sources.
\end{bluebox}


\subsection{Individual Evolution}
\label{Individual Evolution}
Immersed in a dynamic world, individuals mature through an iterative process of memorization, forgetting, error correction, and deepening understanding of the world around them. 
Similarly, LLMs dynamically encapsulate knowledge into parameters through the process of conflict and integration.

In the \textit{pre-training phase}, LLMs start as blank slates, facilitating easier acquisition for new knowledge \cite{DBLP:journals/corr/abs-2404-05405}. Consequently, numerous experiments demonstrate that LLMs accumulate vast amounts of knowledge during this stage \cite{cao-etal-2024-retentive-forgetful,DBLP:conf/nips/ZhouLX0SMMEYYZG23, DBLP:journals/corr/abs-2307-10169, DBLP:journals/corr/abs-2307-06435,DBLP:journals/corr/abs-2212-13138}.
\citet{akyurek2022towards} delve further into identifying which training examples are instrumental in endowing LLMs with specific knowledge.
However, contradictions during the pre-training stage may induce conflicts among internal parametric knowledge.
On the one hand, the false and contradictory information in training corpus propagate and contaminate related memories in LLMs via semantic diffusion, introducing broader detrimental effects beyond direct impacts \cite{Spread}.
On the other hand, LLMs tend to prioritize memorizing more frequent and challenging facts, which can result in subsequent facts overwriting prior memorization, significantly hindering the memorization of low-frequency facts \cite{lu2024scaling}.
In other words, LLMs struggle with balancing and integrating both low and high-frequency knowledge.



After pre-training, LLMs are anticipated to refresh their internal knowledge to keep pace with the evolving world during \textit{post-training stage}. 
Although LLMs seem to absorb new knowledge through continued learning, follow user instructions via instruct tuning \cite{DBLP:journals/corr/abs-2308-10792}, and align with human values through alignment tuning \cite{DBLP:journals/corr/abs-1909-08593}, \citet{ji2024language} have noted that LLMs intrinsically resist alignment during the post-training phase.
In other words, LLMs tend to learn factual knowledge through pre-training, whereas fine-tuning \footnote{Fine-tuning includes instruct tuning and alignment tuning \cite{zhao2023survey}.} teaches them to utilize it more efficiently \cite{DBLP:journals/corr/abs-2405-05904,DBLP:conf/nips/ZhouLX0SMMEYYZG23,ovadia2024finetuning}.
\citet{ren2024learning} also posit that instruction tuning is a form of self-alignment with existing internal knowledge rather than a process of learning new information. 
We conjecture that the debate on whether these processes truly introduce new knowledge stems from information conflicts. For example, the conflict between outdated information within LLMs and new external knowledge exacerbates their difficulty in learning new information.
To mitigate information conflicts, \citet{DBLP:journals/corr/abs-2311-08011} propose first forgetting old knowledge then learning new knowledge.
Another technique, retrieval-augmented generation (RAG) \cite{DBLP:journals/corr/abs-2404-10981}, while avoiding conflicts within internal parameters, still needs to manage conflicts between retrieved external information and LLMs' internal knowledge \cite{DBLP:journals/corr/abs-2403-08319}.
RAG also attempt to efficiently and effectively integrate new knowledge across passages or documents using multiple retrieval \cite{DBLP:journals/corr/abs-2405-13021} and hippocampal indexing \cite{DBLP:journals/corr/abs-2405-14831}.
Besides, editing technologies, including knowledge and representation editing, exhibit promising potential for knowledge addition, modification, and erasure.
Specifically, knowledge editing \cite{ROME,DBLP:conf/iclr/MitchellLBFM22,DBLP:conf/emnlp/CaoAT21,DBLP:journals/corr/abs-2401-01286,DBLP:journals/corr/abs-2310-16218,DBLP:journals/corr/abs-2310-19704} aims to selectively modify model parameters responsible for specific knowledge retention, while representation editing \cite{RepresentationEngineering,ReFT} adjusts the model’s conceptualization of knowledge to revise the stored knowledge within LLMs.
Note that the other strategy for knowledge editing adds external parameters or memory banks for new knowledge while preserving models’ parameters. 
We also provide the comparison of the above methods in \S \ref{appendix:Comparison of Methods for Knowledge Evolution} for better understanding.

\subsection{Group Evolution}
\label{Group Evolution} 

Besides individual learning, social interaction plays a pivotal role in the acquisition of new knowledge and is a key driver of human societal development~\cite{baucalsocial,levine1993social}. 
LLMs, also known as agents, collaborate to accomplish complex tasks during group evolution, each bearing unique knowledge that may sometimes contradict each other.
Therefore, contrary to individual evolution, \textit{group evolution encounters intensified conflicts, such as conflicts in specialized expertise among agents, competing interests, cultural disparities, moral dilemmas, and others}.
To achieve consensus and resolve conflicts, agents must first clarify their own and others' goals (beliefs) through internal representations in models \cite{Beliefs,RepresentationEngineering}.
Agents then discuss, debate, and reflect on shared knowledge through various communication methods \cite{DBLP:conf/iclr/ChanCSYXZF024,DBLP:conf/icml/SmitGDBP24,DBLP:journals/corr/abs-2406-11776,soltoggio2024collective}, e.g., prompt instructions, task and agent descriptions, parameter signals (activation and gradient), and representations of models.
However, conformity of agents, which tends to believe the majority's incorrect answers rather than maintaining their own, hinders conflict resolution during group evolution \cite{jintian-acl,DBLP:conf/www/MaRCS24}.
Note that the group also struggles with automating moral decision-making when facing moral conflicts.
Specifically, agents in the group miss ground truth for moral ``correctness'' and encounter dilemmas due to changes in moral norms over time \cite{DBLP:journals/aiethics/HagendorffD23}.
% Fortunately, we may 
% 一些解决方案
Generally, when, what, and how to share knowledge in the communication process to maximize learning efficiency and long-term expectations are still open questions in group evolution.







Through debate and collaboration, \textit{groups integrate more knowledge and can surpass the cognition of individual units} \cite{debate,chatdev,autoact,multi-agent-coll,jintian-acl}.
This derives from the assumption that each individual unit can contribute to
and benefit from the collective knowledge \cite{soltoggio2024collective,DBLP:journals/corr/abs-2401-11839}.
In addition, \textit{``When a measure becomes a target, it ceases to be a good measure''}, which implies that optimizing one objective on a single individual will inevitably harm other optimization objectives to some extent. 
Hence, it is unrealistic for an individual to learn all knowledge compared to group optimization.
Interestingly, LLM groups also follow the collaborative scaling law \cite{Collaboration}, where normalized solution quality follows a logistic growth pattern as scaling agents.
Moreover, some works \cite{huh2024platonic,Review} propose that knowledge tends to converge into the same representation spaces among the whole artificial neural models group with different data, modalities, and objectives.
% This coexistence of conflict and convergence opens up avenues for the evolution of knowledge within groups of models.




% Agents achieve consensus and resolve conflicts by clarifying their own and others' goals (beliefs), and then sharing their specialized knowledge among each other \citet{soltoggio2024collective}.
% then agents share their knowledge with each other,
% Language Models Represent Beliefs of Self and Others 
% \citet{soltoggio2024collective} further discusses the communication way during knowledge evolution within the model group.


% While there is sufficient theoretical support, we argue that \textbf{the key to group knowledge evolution lies in the forms of knowledge transmission among different LLMs}.
% Humans transmit knowledge through language, images, audio, etc., but these may not necessarily be suitable for machine-to-machine communication.
% For example, information in machines is encoded as embeddings, and whether vectorized embeddings may indeed be a more efficient way for machines to interact is unknown.
% Other potential communication forms include structured text, parameter sharing, memory exchange, etc.
% Furthermore, whether the interaction principles in human-to-human communication are appropriate to machines also needs to be explored.
% 3) Social Science \cite{DBLP:journals/corr/abs-2401-11839}.
% Intuitively, it is precisely due to the accurate division of labor among distinct individuals that the entire human society operates efficiently, which is also applicable to machine society where the individuals are LLMs.
% We explain why group knowledge interaction can achieve higher levels of intelligence based on the following points:
% 1) Information Theory.
% The evolution from a single individual to a group with diverse individuals is a process of entropy increase, which aligns with the principles of development and evolution.
% 2) Goodhart’s Law \citep{goodhart}:
% \textit{``When a measure becomes a target, it ceases to be a good measure''.}
% This implies that optimizing one objective on a single individual will inevitably harm other optimization objectives to some extent.
% This also applies to knowledge evolution which means it is unrealistic for an individual to learn all knowledge.







 

==> cr_section/cr_Introduction.tex <==
\section{Introduction}
\label{Introduction}

Knowledge is the cornerstone of intelligence and the continuation of civilization, furnishing us with foundational principles and guidance for navigating complex problems and emerging challenges \cite{DBLP:journals/aim/DavisSS93,DBLP:conf/wsdm/Choi22}.
Throughout the extensive history of evolution, we have dedicated our lives to cultivating more advanced intelligence by utilizing acquired knowledge and exploring the frontiers of unknown knowledge \cite{DBLP:books/daglib/0067119,DBLP:journals/cacm/HanZL21}.
% However, Knowledge is of no value unless you put it into practice.






As we know, Large language models (LLMs) are renowned for encapsulating extensive parametric knowledge \cite{DBLP:conf/emnlp/RobertsRS20,DBLP:conf/emnlp/SungLYJKK21,DBLP:conf/acl/CaoLHSYLXX20,DBLP:conf/naacl/ZhongFC21,Long-TailKnowledge,DBLP:journals/corr/abs-2008-09036,DBLP:conf/emnlp/PetroniRRLBWM19,DBLP:conf/acl/QiaoO0CYDTHC23,DBLP:conf/kbclm/KritharoulaLS23,DBLP:journals/corr/abs-2402-14273}, achieving unprecedented progress in application.
However, \textit{the knowledge mechanisms in LLMs for learning, storage, utilization, and evolution still remain mysterious} \cite{phillips2021four,DBLP:journals/corr/abs-2312-09230}.
Extensive works aim to demystify various types of knowledge in LLMs through knowledge neurons \cite{KN,chen2024analyzing} and circuits \cite{elhage2021mathematical,knowledgecircuit,CircuitBreakers}, yet these efforts, scattered across various tasks, await comprehensive review and analysis.

\begin{figure}
    \centering
    \includegraphics[width=0.5\textwidth]{fig/framework.png}
    \caption{The analysis framework of knowledge mechanism within neural models includes knowledge evolution and utilization. 
    Dark knowledge denotes knowledge unknown to human or model (machine).
    We investigate the mechanisms of knowledge utilization (right) in LLMs during a specific period of their evolution (left). The knowledge limitations identified through mechanisms analysis will inspire subsequent evolution (left).}
    \label{fig:framwork}
    \vskip -0.1in
\end{figure}


As shown in Fig \ref{fig:framwork}, \textbf{this paper pioneeringly reviews the mechanism across the whole knowledge life cycle.}
We also propose a novel taxonomy for knowledge mechanisms in LLMs,  as illustrated in Fig \ref{taxonomy}, which encompasses knowledge utilization at a specific time and knowledge evolution across all periods of LLMs \footnote{Knowledge utilization focuses on \textit{static} knowledge at a specific period, while knowledge evolution explores the long-term \textit{dynamic} development of knowledge across individual and group LLMs.}.
Specifically, we introduce preliminaries of this field (\S \ref{Preliminary}) and review the knowledge utilization mechanism from a new perspective (\S \ref{Knowledge in LLMs}),
delve into the fundamental principles for knowledge evolution (\S \ref{Knowledge Evolution}).
Then, we investigate how to construct more efficient and trustworthy LLMs from the perspective of knowledge mechanism (\S \ref{Application}).
Later, We discuss open questions about the knowledge LLMs have and have not acquired (\S \ref{Discussion}).
% discuss challenges of knowledge utilization, and posit some promising hypotheses to explore potential avenues for developing powerful and trustworthy models (\S \ref{Discussion}).
Finally, we also provide some future directions (\S \ref{Future_Directions}) and tools for knowledge mechanism analysis (\S \ref{appendix:Tools}).
Our contributions are as follows:
% Generally, 


% Later, we will discuss the knowledge LLMs have acquired, the reasons for its fragility, the characteristics of unlearned dark knowledge, and strategies for continuously expanding the boundaries of this dark knowledge.

\input{fig/taxonomy}



\begin{itemize}[leftmargin=*,nosep]
    \item To the best of our knowledge, we are the first to review knowledge mechanisms in LLMs and provide \textbf{a novel taxonomy} across the entire life.
    \item We propose a new perspective to analyze knowledge utilization mechanisms from \textbf{three levels: memorization, comprehension and application, and creation}.
    \item We discuss \textbf{knowledge evolution} in individual and group LLMs, and analyze the inherent conflicts and integration in this process.
    \item We observe that LLMs have learned basic world knowledge. However, the learned knowledge is fragile, leading to challenges such as \textbf{hallucinations and knowledge conflicts}. We speculate that this fragility may be primarily due to improper learning data. Besides, the unlearned \textbf{dark knowledge} will exist long.
   %  \item We suspect that the prevalent transformer architecture may impede creativity, data distribution and quantity may contribute to the fragility of parametric knowledge, leading \textbf{hallucinations and knowledge conflict}.
   % Besides, \textbf{dark knowledge} will exist for a long time.
\end{itemize}


\paragraph{Comparison with Existing Surveys}
Previous interpretability surveys typically aim to investigate various \textit{methods for explaining the roles of different components} within LLMs from the global and local taxonomy \cite{DBLP:journals/corr/abs-2405-00208,DBLP:journals/tist/ZhaoCYLDCWYD24,DBLP:journals/corr/abs-2401-12874,DBLP:journals/corr/abs-1901-04592,PracticalReview,Review,PositionPaper,DBLP:journals/corr/abs-2402-01761}.
In contrast, this paper focuses on knowledge in LLMs.
Hence, \textit{our taxonomy, oriented from target knowledge in LLMs, reviews how knowledge is acquired, stored, utilized, and subsequently evolves}.
Additionally, previous taxonomy mostly explore the explainability \textit{during the inference stage} (a specific period), while ignoring knowledge acquisition during the pre-training stage and evolution during the post-training stage \cite{DBLP:conf/satml/RaukerHCH23,DBLP:journals/csur/LuoIHP24,DBLP:journals/coling/Apidianaki23,DBLP:journals/staeors/JiaoHLYMZYHYLMLCFTGZQWLBLSF23,DBLP:conf/satml/RaukerHCH23,rai2024practical}.
Our taxonomy aims to explore the \textit{dynamic evolution across all periods} from naivety to sophistication in both individual and group LLMs.
In contrast to the most similar survey \cite{DBLP:journals/ijautcomp/CaoLHS24} that introduces knowledge life cycle, our work focuses on the underlying mechanisms at each stage. 










Generally, this paper may help us to explore and manipulate advanced knowledge in LLMs, examine current limitations through the history of knowledge evolution, and \textbf{inspire more efficient and trustworthy architecture and learning strategy for future models from knowledge mechanism perspective}.
Note that most hypotheses in this paper are derived from transformer-based LLMs.  
We also validate the generalizability of these hypotheses across other architectural models and then propose universality intelligence in \S \ref{appendix:Universality Intelligence}.

% Fortunately, artificial neural models tend to exhibit universal intelligence \cite{huh2024platonic}.

% similar conclusions are also observed in other architectures, which are detailed

% and review the processes of knowledge evolution among the artificial neural models group.

% Note that most hypotheses in this paper are derived from transformer-based models.
% Fortunately, artificial neural models may tend to universality intelligence \cite{huh2024platonic} and 
% we validate the generalizability of these hypotheses across other architectures models in \S \ref{appendix:Universality Intelligence}.

% focus on behavior explainability during the inference stage, while ignoring knowledge acquisition during the pre-training stage and evolution during the post-training stage \cite{DBLP:journals/corr/abs-2401-12874,DBLP:journals/corr/abs-2405-00208,DBLP:journals/tist/ZhaoCYLDCWYD24,DBLP:journals/corr/abs-1901-04592,Review,PositionPaper,DBLP:journals/corr/abs-2402-01761,DBLP:conf/satml/RaukerHCH23,DBLP:journals/csur/LuoIHP24,DBLP:journals/coling/Apidianaki23,DBLP:journals/staeors/JiaoHLYMZYHYLMLCFTGZQWLBLSF23,DBLP:conf/satml/RaukerHCH23,rai2024practical}.
% In contrast to the most similar survey \cite{DBLP:journals/ijautcomp/CaoLHS24} that introduces knowledge life cycle, our work focuses on the underlying mechanisms at each stage. 












% 相比于我们最像的研究xx介绍了knowledge life cycle，我们关注的是每个阶段的底层机理分析，首次分析了知识创造和群体知识演化的过程。

% local and global 
% \cite{DBLP:journals/corr/abs-2309-01029, DBLP:journals/corr/abs-2401-12874, DBLP:journals/aamas/RosenfeldR19, DBLP:journals/corr/abs-1901-04592,DBLP:journals/information/AlangariMMA23a} primarily focus on the information and skills that LLMs already possess during the inference stage. In contrast, this paper delves into the knowledge storage, application, and evolution in LLMs across inference and \todo{post-training} stages.



% % 列几个相关survey  1 ）知识自身survey  

% %下列论文都要cite

% Language models as knowledge bases?

% A review on language models as knowledge bases



% Language models as knowledge bases: On entity representations, storage capacity, and paraphrased queries





% Revealing the Parametric Knowledge of Language Models:
% A Unified Framework for Attribution Methods
% %2） 可解释survey

% %自己加

==> cr_section/cr_Knowledge_Representation.tex <==

\section{Knowledge Utilization in LLMs}
\label{Knowledge in LLMs}

We introduce some preliminaey in \S \ref{Preliminary}, including the definition of knowledge in LLMs and knowledge analysis methods.
Then, inspried by Bloom's Taxonomy of cognition levels \cite{wilson2016anderson,bloom1956taxonomy,keene2010mapping,fadul2009collective}, we categorize knowledge representation and utilization within LLMs into three levels (as shown in Fig \ref{fig:utilization}): memorization, comprehension and application, and creation \footnote{
Note that we combine analyzing, evaluating, and creating from Bloom's Taxonomy into one category level (creation) in our taxonomy, as they are difficult to disentangle.
Specifically, creation emphasizes the capacity and process of forming \textit{novel} and \textit{valuable} things. 
Analyzing \cite{wilson2016anderson}, which breaks materials or concepts into parts, is used for creating \textit{novel} things.
Evaluating \cite{wilson2016anderson} is usually used for assessing the \textit{value} of new creations.}.
% We review related work in Fig \ref{taxonomy}
% as shown in Fig \ref{fig:utilization}, 
% This section delves into mechanisms across the above levels, respectively.
Note that these mechanistic analyses are implemented via methods in \S \ref{Methods of Knowledge Analysis}.
We further evaluate the applicability, advantages, and limitations of different methods in \S \ref{Comparison of Different Analysis Methods}.




\begin{figure}[!t]
    \centering
    \includegraphics[width=0.5\textwidth]{fig/new-utilization.png}
    \caption{The mechanism analysis for knowledge utilization across three levels: memorization, comprehension and application, and creation.}
    \label{fig:utilization}
    \vskip -0.15in
\end{figure}


\subsection{Memorization}
\label{Memorization}
Knowledge memorization \cite{DBLP:journals/corr/abs-2404-15146,MultifacetedMemorization} aims to remember and recall knowledge in the training corpus, e.g.,  specific terms (entities), grammar, facts, commonsense, concepts, etc \cite{DBLP:journals/corr/abs-2305-13673,DBLP:journals/corr/abs-2306-09296,DBLP:journals/corr/abs-2301-06627,DBLP:journals/corr/abs-2309-14316,DBLP:journals/corr/abs-2309-14402,DBLP:journals/corr/abs-2404-05405,DBLP:journals/ijautcomp/CaoLHS24}.
\textit{We posit knowledge memorization from Modular Region and Connection Hypothesis by reviewing existing research.}



\begin{bluebox}[Hypothesis 1: Modular Region]
Knowledge is Encoded in Modular Regions.
\label{Hypothesis 1}
\end{bluebox}

This modular region hypothesis simplifies knowledge representation in transformer-based models into isolated modular region, e.g., MLPs or {attention heads}.
\textbf{Knowledge is encoded via MLPs.} \citet{Key-ValueMemories} posit that MLPs operate as key-value memories and each individual key vector corresponds to a specific \textit{semantic pattern} or \textit{grammar}.
Based on the above finding, \citet{DBLP:conf/emnlp/GevaCWG22,LM-Debugger} reverse engineer the operation of the MLPs layers and find that MLPs can promote both {semantic} (e.g., measurement semantic including kg, percent, spread, total, yards, pounds, and hours) and \textit{syntactic} (e.g., adverbs syntactic including largely, rapidly, effectively, previously, and normally) {concepts} in the vocabulary space.
\citet{An} find a single MLP neuron (in GPT-2 Large) capable of generating ``an'' or ``a''.
Subsequently, \textit{fact} \cite{KN,ROME} and \textit{commonsense} knowledge \cite{DBLP:conf/emnlp/GuptaMS00WT23} are found. 
Advanced language-specific neurons \cite{Language-Specific}, linguistic regions \cite{functionregion}, entropy neurons \cite{stolfo2024confidence}, abstract conceptual \cite{ConceptEdit} and unsafe \cite{DINM,DBLP:conf/emnlp/WuLXDW0X23} knowledge, are also observed in MLPs.
In addition to MLP, \textbf{knowledge is also conveyed by attention heads} \cite{geva-etal-2023-dissecting,SuccessorHeads}.
\citet{DBLP:conf/acl/HooverSG20} explain the knowledge each attention head has learned. Specifically, attention heads store evident \textit{linguistic features, positional information}, and so on.
Besides, \textit{fact knowledge} \cite{Characterizing,DBLP:conf/nips/0002PVPW23} and \textit{bias} \cite{DBLP:conf/acl/HooverSG20} are mainly convey by attention heads.
\citet{dreamofelephants} further observe that LLMs leverage self-attention to gather information through certain tokens in the contexts, which serve as clues, and use the value matrix for associative memory.
Later, \citet{Beliefs} also find that attention heads can simulate \textit{mental stat}e and activate ``Theory of Mind'' (ToM) capability.



However, Hypothesis 1 ignores the connections between different regions.
Inspired by advancements in neuroscience \cite{thiebaut2022emergent}, Hypothesis 2 asserts that the connection of different components integrates knowledge, rather than the isolated regions in Hypothesis 1.

 % also claim that some attention heads can trigger the ability of in-context-learning
% \paragraph{Additionally, knowledge may be situated in hybrid regions, including MLPs and attention heads.}

\begin{bluebox}[Hypothesis 2: Connection]
Knowledge is Represented by Connections.
\end{bluebox}

% Generally, fact knowledge, e.g., ``The capital of Ireland is Dublin'', can be expressed as triplet, e.g., (Ireland, capital of, Dublin).
\citet{geva-etal-2023-dissecting} outline the encoding of factual knowledge (e.g., ``The capital of Ireland is Dublin'') through the following three steps: (1) subject (Ireland) information enrichment in MLPs, (2) the relation (capital of) propagates to the last token, (3) object (Dublin) is extracted by attention heads in later layers.
This claim is supported by \citet{PMET}.
Similarly, \citet{DBLP:journals/corr/abs-2403-19521} conclude that task-specific attention head may move the topic entity to the final position of the residual stream, while MLPs conduct relation function.
Moreover, the recent prominent knowledge circuit framework \cite{DBLP:journals/corr/abs-2401-03646,knowledgecircuit,DBLP:journals/corr/abs-2402-12201,elhage2021mathematical,DBLP:journals/corr/abs-2403-19647} advocates leveraging a critical computational subgraph among all components to explore internal knowledge within LLM parameters.
The competencies for indirect object identification and color object tasks are discovered to be embedded in specialized knowledge circuits \cite{ACDC,WangVCSS23,DBLP:journals/corr/abs-2310-08744,yu2024functional}.
\citet{SharedCircuits} also identify number-related circuits that encode the predictive ability of Arabic numerals, number words, and months.
More importantly, experimental evidence demonstrates that various types of knowledge, including linguistic, commonsense, factual, and biased information, are encapsulated in specific knowledge circuits \cite{knowledgecircuit}.
Interestingly, knowledge encoded by specific circuits can rival or even surpass that of the entire LLM.
This may be because knowledge circuits memorized the relevant knowledge, while noise from other components might impede the model's performance on these tasks.


% within the neural network.



\subsection{Comprehension and Application}
\label{Comprehension and Application}
Knowledge comprehension and application focus on demonstrating the understanding of memorized knowledge and then solving problems in new situations, e.g., \textit{generalization on out-of-domain tasks} \cite{Grokked}, \textit{reasoning \cite{DBLP:conf/emnlp/HouLFSZZBS23} and planning} \cite{ChessKnowledge}.
\citet{DBLP:journals/corr/abs-2303-11873} denote the transition from memorization to comprehension and application as grokking, and suggest that the grokking derives from two largely distinct subnetworks competition.
Intuitively, only knowledge that is correctly memorized \cite{MultifacetedMemorization} in \S \ref{Memorization} can be further applied to solving complex tasks.
Therefore, we posit the following Reuse Hypothesis from two knowledge memorization perspectives.


\begin{bluebox}[Hypothesis 3: Reuse]
LLMs Reuse Certain Components during Knowledge Comprehension and Application.
\end{bluebox}

\textbf{From the Modular Region Perspective, knowledge utilization reuses some regions.}
These regions might include a few neurons, attention heads, MLPs, a transformer layer, or partial knowledge circuits.
Generally, basic knowledge (position information, n-gram pattern, syntactic features) tends to be stored at earlier layers, while sophisticated knowledge (mental state, emotion, and abstract concept, e.g., prime number, Camelidae, and safety) is located at later layers \cite{Beliefs,DBLP:journals/corr/abs-2404-07066,DINM,ConceptEdit,ShortGPT,kobayashi2023analyzing}. 
Therefore, \textit{neurons of earlier layers related to basic knowledge tend to be reused} \cite{DBLP:conf/emnlp/KangC23,DBLP:journals/tist/ZhaoCYLDCWYD24,Long-TailKnowledge}.
Various math reasoning tasks also utilize the attention mechanism in initial layers to map input information to the final token positions, subsequently generating answers using a set of MLPs in later layers \cite{DBLP:conf/emnlp/StolfoBS23,mathematical,DecoderLens}.
Besides, \textit{some specific function regions are also reused}.
Specifically, retrieval heads \cite{DBLP:conf/nips/0002PVPW23} are reused for Chain-of-Thought (CoT) reasoning and long-context tasks. These retrieval heads are found in 4 model families, 6 model scales, and 3 types of fine-tuning.
Subsequently, induction heads, identified in Llama and GPT, are claimed to be reused for in-context learning (ICL) tasks \citet{InductionHeads,InductionHeadsPattern}.
Attention heads can map country names to their capitals in capital city-related tasks \cite{DBLP:journals/corr/abs-2403-19521}. 
% \citet{DBLP:conf/nips/0002PVPW23} demonstrate that some attention heads (in Alpaca, Llama, and Vicuna) exhibit the capability for truthful answers instead of hallucinations.
Language-specific neurons (in Llama and BLOOM) are responsible for multiple language related tasks, such as English, French, Mandarin, and others \citet{Language-Specific}.
\citet{functionregion} further reveal linguistic regions (in Llama) correspond to linguistic competence, which is the cornerstone for performing various tasks.
Later, function regions related to the process of math reasoning are also discovered in LLMs.
For instance, the last layer of GPT-2 (trained from scratch) has been observed to exhibit mathematical reasoning abilities across various math questions \cite{Part2.1}.
\textbf{From the Connection Perspective, knowledge utilization shares partial knowledge circuits.}
For instance, similar tasks share subgraphs (computational circuits) with analogous roles \cite{SharedCircuits}.
Besides, knowledge circuits (in GPT2) are reused to solve a seemingly different task, e.g., indirect object identification and colored objects tasks \cite{DBLP:journals/corr/abs-2310-08744}.
\citet{Grokked} further observe that two-hop composition reasoning tasks reuse the knowledge circuits from the first hop. 
\citet{knowledgecircuit} also believe that this reuse phenomenon exists in factual recall and multi-hop reasoning. Specifically, sub-circuits are reused in similar factual knowledge, such as tasks related to ``city\_in\_country'', ``name\_birth\_place'', and ``country\_language''.
Besides, \citet{DBLP:journals/corr/abs-2402-18312} demystify LLMs how to perform CoT reasoning, i.e., Llama facilitates CoT tasks via multiple parallel circuits enjoying significant intersection.







\subsection{Creation}
\label{Creation}
Knowledge creation \cite{runco2012standard,sternberg2006nature} emphasizes the capacity and process of forming \textit{novel} and \textit{valuable} things, rather than the existing ones (i.e., LLMs have seen) discussed in \S \ref{Memorization} and \S \ref{Comprehension and Application}.
The creations encompass two levels:
1) LLMs create new terms following the current world's principles comprehended by LLMs, such as new proteins \cite{Shin_Riesselman_Kollasch_McMahon_Simon_Sander_Manglik_Kruse_Marks_2021}, molecules \cite{DBLP:journals/jcisd/BagalAVP22,DBLP:journals/corr/abs-2301-11259,DBLP:conf/emnlp/EdwardsLRHCJ22}, code \cite{DBLP:journals/corr/abs-2404-08806}, video \cite{DBLP:journals/corr/abs-2312-14125}, models \cite{DBLP:journals/corr/abs-2404-16792}, names for people and companies, written stories \cite{DBLP:journals/corr/abs-2405-13012,DBLP:conf/emnlp/Gomez-Rodriguez23a,DBLP:journals/corr/abs-2405-01660}, synthetic data \cite{DBLP:journals/jbd/StengerLFKB24,DBLP:journals/corr/abs-2403-10075,DBLP:conf/acit3/AbufaddaM21}, etc.
These novel items operate according to the existing rules, e.g., law of conservation of energy, reasoning logic \cite{Grokked}, or principles of probability theory.
2) LLMs may generate new rules, such as mathematical theorems, and the resulting terms will operate according to the new rules.
We posit that the knowledge creation of LLMs may derive from the Extrapolation Hypothesis.
% 数学公式 新的定理 

\begin{bluebox}[Hypothesis 4: Extrapolation]
LLMs May Create Knowledge via Extrapolation.
\end{bluebox}

% From a distributional perspective, the operational principles of the current world can be viewed as a \todo{continuous distribution}, while the knowledge we currently observe consists of discrete, finite points within this distribution 
The expression of knowledge is diverse; some knowledge is inherently continuous. Therefore, it is difficult, if not impossible, to represent certain knowledge using discrete data points \cite{continuity,penroselimitations,markman2013knowledge}. 
LLMs utilize insights into the operational principles of the world to extrapolate additional knowledge from known discrete points, bridging gaps in knowledge and expanding our understanding of the world\cite{heilman2003creative,DBLP:journals/corr/abs-2401-17692,DBLP:journals/corr/abs-2311-03658,DBLP:journals/corr/abs-2312-14125}.
Drawing inspiration from research on human creativity \cite{DBLP:journals/corr/abs-2303-12003}, the \textit{physical implementation of knowledge extrapolation relies on the plasticity of neurons} \cite{DBLP:journals/corr/abs-2404-04436}. 
Specifically, plasticity refers to LLMs changing activations and connectivity between neurons according to the input \cite{Gaming}.

However, from statistical perspective, the intricate connections and activations between neurons, though not infinite, resist exhaustive enumeration. In terms of value, not all creations are valuable. 
Obtaining something valuable with an exceedingly low probability is impractical, as even a monkey could theoretically print Shakespeare's works.
How do LLMs ensure the probability of generating valuable creations? 
\textit{What are the mechanisms underlying the novelty and value of creation?}
A prevalent conjecture posits that \textbf{novelty is generated through the random walk} \cite{DBLP:journals/corr/abs-2403-06996}.
However, intuitively, \textbf{current LLMs themselves seem unable to evaluate the value of creations due to architectural limitations} \cite{DBLP:conf/chi/ChakrabartyLAMW24}. 
Because, once the next token is generated, there is no intrinsic mechanism for accepting or rejecting the creations. This hinders the evaluation of the usefulness and value of proposed novelties, as humans do, by bending, blending, or breaking biases \cite{DBLP:journals/corr/abs-2403-06996}.
Some works assume that each token is indeed valuable and meets long-term expectations.
However, the well-known hallucination problem \cite{DBLP:journals/corr/abs-2401-11817} of LLMs refutes this assumption.
% This will be further discussed in \S \ref{Dark Knowledge}.
Besides, the transformer architecture struggles with long context \cite{DBLP:journals/corr/abs-2404-02060}, despite the existence of many variants for addressing this issue \cite{DBLP:journals/corr/abs-2311-12351,InfiniteContext}.
% 无法处理长文本，面对长文本时倾向于复制。
More importantly, MLPs of Transformer may also work contrary to creativity, i.e., the increased attentions narrow the conditional distribution for token prediction \cite{DBLP:journals/corr/abs-2403-06996}.














